Decomposition of Global Feature Importance into Direct and Associative Components (DEDACT)

Global model-agnostic feature importance measures either quantify whether features are directly used for a model's predictions (direct importance) or whether they contain prediction-relevant information (associative importance). Direct importance provides causal insight into the model's mechanism, yet it fails to expose the leakage of information from associated but not directly used variables. In contrast, associative importance exposes information leakage but does not provide causal insight into the model's mechanism. We introduce DEDACT - a framework to decompose well-established direct and associative importance measures into their respective associative and direct components. DEDACT provides insight into both the sources of prediction-relevant information in the data and the direct and indirect feature pathways by which the information enters the model. We demonstrate the method's usefulness on simulated examples.

==> figures/further_decomposition_experiments/wbars_cause_and_effect.tex <==
\begin{figure}[H]
\centering
\subfigure[DAG Cause and Effect]{
\begin{tikzpicture}[thick, scale=.65, every node/.style={scale=.68, line width=0.25mm, black, fill=white}]

		\node[draw, circle, scale=0.7] (x1) at (0, 1) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (x3) at (0,-1) {$X_3$};
		\node[draw, circle, scale=0.7] (x4) at (0,-2) {$X_4$};
		\node[draw, circle, scale=0.7] (y) at (-1.25,-0.5) {$Y$};
		\draw[dashed,gray] (-1.6,-2.35) -- (.35,-2.35) -- (.35,1.35) -- (-1.6,1.35) -- cycle;
		\node[scale=0.7] (dots) at (-.625,-2.6) {data};
		\draw[->] (x1) -- (x2);
		\draw[->] (x2) -- (y);
		\draw[->] (y) -- (x3);
		\draw[->] (x3) -- (x4);
		
		
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (ux3) at (1,-1) {$\underline{X}_3$};
		\node[draw, circle, scale=0.7] (ux4) at (1,-2) {$\underline{X}_4$};
		\draw[dashed,gray] (0.65,-2.35) -- (2.35,-2.35) -- (2.35,1.35) -- (0.65,1.35) -- cycle;
		\node[scale=0.7] (dots) at (1.5,-2.6) {model};
		\draw[->] (x1) -- (ux1);
		\draw[->] (x2) -- (ux2);
		\draw[->] (x3) -- (ux3);
		\draw[->] (x4) -- (ux4);

		\node[draw, circle, scale=0.7] (yhat) at (2, -.5) {$\hat{Y}$};
		\draw[->] (ux2) -- (yhat);
		\draw[->] (ux3) -- (yhat);

\end{tikzpicture}
}
\subfigure[Results TDI decomp]{
    \includegraphics[width=0.75\linewidth]{figures/wbars_ii-cause_and_effect_unordered_rfi_decomp.pdf}
}
\subfigure[Results TAI decomp]{
    \includegraphics[width=\linewidth]{figures/wbars_ii-cause_and_effect_tai_decomp_unordered.pdf}
}
\subfigure[Results TAI decomp naive]{
    \includegraphics[width=\linewidth]{figures/wbars_ii-cause_and_effect_tai_decomp_unordered_naive.pdf}
}
%
\caption{Cause and Effect Results}
\label{fig:dag-cause-and-effect}
\end{figure}

==> figures/further_decomposition_experiments/wbars_inference_large.tex <==
\begin{figure}[H]
\centering
\subfigure[DAG Two Causes]{
\begin{tikzpicture}[thick, scale=.65, every node/.style={scale=.68, line width=0.25mm, black, fill=white}]

		\node[draw, circle, scale=0.7] (x1) at (0, 1) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (x3) at (0,-1) {$X_3$};
		\node[draw, circle, scale=0.7] (x4) at (0,-2) {$X_4$};
		\node[draw, circle, scale=0.7] (y) at (-1.25,-0.5) {$Y$};
		\draw[dashed,gray] (-1.6,-2.35) -- (.35,-2.35) -- (.35,1.35) -- (-1.6,1.35) -- cycle;
		\node[scale=0.7] (dots) at (-.625,-2.6) {data};
		\draw[->] (x1) -- (x2);
		\draw[->] (x2) -- (y);
		\draw[->] (x4) -- (x3);
		\draw[->] (x3) -- (y);
		
		
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (ux3) at (1,-1) {$\underline{X}_3$};
		\node[draw, circle, scale=0.7] (ux4) at (1,-2) {$\underline{X}_4$};
		\draw[dashed,gray] (0.65,-2.35) -- (2.35,-2.35) -- (2.35,1.35) -- (0.65,1.35) -- cycle;
		\node[scale=0.7] (dots) at (1.5,-2.6) {model};
		\draw[->] (x1) -- (ux1);
		\draw[->] (x2) -- (ux2);
		\draw[->] (x3) -- (ux3);
		\draw[->] (x4) -- (ux4);

		\node[draw, circle, scale=0.7] (yhat) at (2, -.5) {$\hat{Y}$};
		\draw[->] (ux2) -- (yhat);
		\draw[->] (ux3) -- (yhat);

\end{tikzpicture}
}
\subfigure[TDI Decomposition]{
    \includegraphics[width=0.75\linewidth]{figures/wbars_ii-inference-large_unordered_rfi_decomp.pdf}
}
\subfigure[TAI Decomposition]{
    \includegraphics[width=\linewidth]{figures/wbars_ii-inference-large_tai_decomp_unordered.pdf}
}
\subfigure[TAI Decomposition Naive]{
    \includegraphics[width=\linewidth]{figures/wbars_ii-inference-large_tai_decomp_unordered_naive.pdf}
}
%
\caption{II Inference Large results}
\label{fig:dag-ii-inference-large} 
\end{figure}

==> figures/further_decomposition_experiments/wbars_rhombus.tex <==
\begin{figure}[H]
\centering
\subfigure[DAG Rhombus]{
\begin{tikzpicture}[thick, scale=.65, every node/.style={scale=.68, line width=0.25mm, black, fill=white}]

		\node[draw, circle, scale=0.7] (x1) at (0, 1) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (-1.25, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (x3) at (0,-1) {$X_3$};
		\node[draw, circle, scale=0.7] (y) at (-1.25,-2) {$Y$};
		\draw[dashed,gray] (-1.6,-2.35) -- (.35,-2.35) -- (.35,1.35) -- (-1.6,1.35) -- cycle;
		\node[scale=0.7] (dots) at (-.625,-2.6) {data};
		\draw[->] (x1) -- (x2);
		\draw[->] (x1) -- (x3);
		\draw[->] (x2) -- (y);
		\draw[->] (x3) -- (y);
		
		
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (ux3) at (1,-1) {$\underline{X}_3$};
		\draw[dashed,gray] (0.65,-2.35) -- (2.35,-2.35) -- (2.35,1.35) -- (0.65,1.35) -- cycle;
		\node[scale=0.7] (dots) at (1.5,-2.6) {model};
		\draw[->] (x1) -- (ux1);
		\draw[->] (x2) -- (ux2);
		\draw[->] (x3) -- (ux3);

		\node[draw, circle, scale=0.7] (yhat) at (2, 0) {$\hat{Y}$};
		\draw[->] (ux2) -- (yhat);
		\draw[->] (ux3) -- (yhat);

\end{tikzpicture}
}
\subfigure[TDI decomposition]{
    \includegraphics[width=0.75\linewidth]{figures/wbars_ii-cause_and_effect_unordered_rfi_decomp.pdf}
}
\subfigure[TAI decomposition]{
    \includegraphics[width=\linewidth]{figures/wbars_ii-cause_and_effect_tai_decomp_unordered.pdf}
}
\subfigure[TAI decomposition naive]{
    \includegraphics[width=\linewidth]{figures/wbars_ii-cause_and_effect_tai_decomp_unordered_naive.pdf}
}
%
\caption{Rhombus results}
\label{fig:dag-rhombus} 
\end{figure}

==> figures/old/dag-audit-example.tex <==
\begin{figure}[!htb]
\centering
\subfigure[PFI]{
\includegraphics[width=0.25\textwidth]{figures/example-audit-fi}
}
\subfigure[SI]{
\includegraphics[width=0.25\textwidth]{figures/example-audit-si}
}
\subfigure[DAG]{
	\begin{tikzpicture}[thick, scale=1.4, every node/.style={scale=0.8, line width=0.3mm, black, fill=white}]
		%

		\draw[dotted] (-1.3,-.25) -- (.3,-.25) -- (.3,1.25) -- (-1.3,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (x1) at (0, 1.) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (y) at (-1, .5) {$Y$};
		\node[scale=0.7] (dots) at (-.5, -.5) {data level, variables};
		
		\draw[dotted] (.7,-.25) -- (2.3,-.25) -- (2.3,1.25) -- (.7,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (yhat) at (2, .5) {$\hat{Y}$};
		\node[scale=0.7] (dots) at (1.5,-.5) {model level, features};
		
		\draw[->] (x1) -- (y);
		\draw[->] (x1) -- (x2);
		\draw[->] (x1) -- (ux1);
		\draw[->] (x2) -- (ux2);
		\draw[->] (ux2) -- (yhat);
	
	\end{tikzpicture}
	
}

\caption{A linear OLS regression model was fit on $D = \{X_1, X_2\}$ to predict $Y$. (a) Permutation Feature Importance for $X_1$ and $X_2$. We can see that $X_1$ is not directly being used by the model, wheras $X_2$ is directly being used. We cannot see the indirect influence of $X_1$. (b) We see that both variables, $X_1$ and $X_2$, are associated with the prediction performance. However, we do not know via which feature the association enters the model. (c) \textit{Left:} A causal DAG depicting the underlying data generating mechanism. Variable $X_1$ causes both $Y$ and $X_2$. As a consequence $Y$ and $X_2$ are dependent. \textit{Right:} A DAG depicting the Structural Causal Model of the prediction function $f$. The model $f$ only relies on a measurement of $X_2$, here denoted as $\underline{X}_2$, for its predictions. Although the feature $\underline{X}_1$ is not directly being used by the model, the prediction $\hat{Y}$ depends on $X_1$ via variable $X_2$. }
\label{fig:dag-audit-example} 

\end{figure}

==> figures/old/dag-inference-example-large.tex <==
\begin{figure}[h]
\centering
%
%\subfigure[PFI]{
%	\includegraphics[width=0.25\textwidth]{figures/example-inference-large-fi}
%}
%
%\subfigure[SI]{
%	\includegraphics[width=0.25\textwidth]{figures/example-inference-large-si}
%}
%
\subfigure[Decomposition]{
    \includegraphics[width=0.65\textwidth]{figures/ii_inference_large.pdf}
}
%
\subfigure[DAG]{
		\begin{tikzpicture}[thick, scale=0.8, every node/.style={scale=0.8, line width=0.3mm, black, fill=white}]
		%

		\draw[dotted] (-1.3,-1.25) -- (.3,-1.25) -- (.3,2.25) -- (-1.3,2.25) -- cycle;
		\node[draw, circle, scale=0.7] (x1) at (0, 2.) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 1) {$X_2$};
		\node[draw, circle, scale=0.7] (x3) at (0, 0.) {$X_3$};
		\node[draw, circle, scale=0.7] (x4) at (0, -1) {$X_4$};
		\node[draw, circle, scale=0.7] (y) at (-1, .5) {$Y$};tt
		\node[scale=0.7] (dots) at (-.5, -1.5) {data level, variables};
		
		\draw[dotted] (.7,-1.25) -- (2.3,-1.25) -- (2.3,2.25) -- (.7,2.25) -- cycle;
		\node[draw, circle, scale=0.7] (ux1) at (1, 2) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 1) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (ux3) at (1, 0) {$\underline{X}_3$};
		\node[draw, circle, scale=0.7] (ux4) at (1, -1) {$\underline{X}_4$};
		\node[draw, circle, scale=0.7] (yhat) at (2, .5) {$\hat{Y}$};
		\node[scale=0.7] (dots) at (1.5,-1.5) {model level, features};
		
		\draw[->] (x2) -- (y);
		\draw[->] (x1) -- (x2);
		\draw[->] (x4) -- (x3);
		\draw[->] (x3) -- (y);
		\draw[->, dashed] (x1) -- (ux1);
		\draw[->, dashed] (x2) -- (ux2);
		\draw[->, dashed] (x3) -- (ux3);
		\draw[->, dashed] (x4) -- (ux4);
		\draw[->] (ux2) -- (yhat);
		\draw[->] (ux3) -- (yhat);
	
		\end{tikzpicture}	
}
%
\caption{We decomposed the PFI for a model fit on the dataset above. The model relies directly on $\underline{X}_2, \underline{X}_3$, but not on $\underline{X}_1, \underline{X}_4$. However $X_1$ and $X_4$ indirectly influence the prediction via $X_2$ and $X_3$ respectively, which can be seen in (a).}

\label{fig:dag-inference-example} 

\end{figure}

==> figures/old/dag-inference-example.tex <==
\begin{figure}[h]
\centering
%
\subfigure[PFI]{
	\includegraphics[width=0.25\textwidth]{figures/example-inference-fi}
}
%
\subfigure[SI]{
	\includegraphics[width=0.25\textwidth]{figures/example-inference-si}
}
%
\subfigure[DAG]{
		\begin{tikzpicture}[thick, scale=1.4, every node/.style={scale=0.8, line width=0.3mm, black, fill=white}]
		%

		\draw[dotted] (-1.3,-.25) -- (.3,-.25) -- (.3,1.25) -- (-1.3,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (x1) at (0, 1.) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (y) at (-1, .5) {$Y$};tt
		\node[scale=0.7] (dots) at (-.5, -.5) {data level, variables};
		
		\draw[dotted] (.7,-.25) -- (2.3,-.25) -- (2.3,1.25) -- (.7,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (yhat) at (2, .5) {$\hat{Y}$};
		\node[scale=0.7] (dots) at (1.5,-.5) {model level, features};
		
		\draw[->] (x2) -- (y);
		\draw[->] (x1) -- (x2);
		\draw[->] (x1) -- (ux1);
		\draw[->] (x2) -- (ux2);
		\draw[->] (ux2) -- (yhat);
	
		\end{tikzpicture}	
}
%
\caption{(a)Permutation Feature Importance. Feature Importance for $X_1$ is zero, therefore the variable is not used by the model. (b) Shared Information: $X_1$ is associated with the prediction performance. (c) \textit{Left:} A causal DAG depicting the underlying data generating mechanism. Variable $X_1$ causes $X_2$ and $X_2$ causes $Y$. As a consequence $Y$ and $X_1$ are dependent. \textit{Right:} A DAG depicting the Structural Causal Model of the prediction function $f$. The model $f$ only relies on a measurement of $X_2$, here denoted as $\underline{X}_2$, for its predictions. Although the feature $\underline{X}_1$ is not directly being used by the model, the prediction $\hat{Y}$ depends on $X_1$ via variable $X_2$.}

\label{fig:dag-inference-example} 

\end{figure}

==> figures/old/dag-motivation-old.tex <==
\begin{figure}[!htb]
\centering
\subfigure[DAG]{
	\begin{tikzpicture}[thick, scale=1.3, every node/.style={scale=0.8, line width=0.3mm, black, fill=white}]
		%

		\draw[dotted] (-1.3,-1.25) -- (.3,-1.25) -- (.3,1.25) -- (-1.3,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (x1) at (0, 1) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (x3) at (0, -1) {$X_3$};
		\node[draw, circle, scale=0.7] (y) at (-1, .5) {$Y$};
		\node[scale=0.7] (dots) at (-.5, -1.5) {data level, variables};
		
		\draw[dotted] (.7,-1.25) -- (2.3,-1.25) -- (2.3,1.25) -- (.7,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (ux3) at (1, -1) {$\underline{X}_3$};
		\node[draw, circle, scale=0.7] (yhat) at (2, .5) {$\hat{Y}$};
		\node[scale=0.7] (dots) at (1.5,-1.5) {model level, features};
		
		\draw[->] (x1) -- (y);
		\draw[->] (x2) -- (y);
		\draw[->] (x2) -- (x3);
		\draw[->,gray] (x1) -- (ux1);
		\draw[->,gray] (x2) -- (ux2);
		\draw[->,gray] (x3) -- (ux3);
		\draw[->] (ux1) -- (yhat);
		\draw[->] (ux2) -- (yhat);
	
	\end{tikzpicture}
	
}
\subfigure[Direct and Total (obs.) Importance]{
\includegraphics[width=0.5\textwidth]{figures/relevance_types_direct_vs_total}
}
\caption{A linear OLS regression model was fit on $D = \{X_1, X_2, X_3\}$ to predict $Y$. (a) \textit{Left:} A causal DAG depicting the underlying data generating mechanism. All relationships are linear with Gaussian noise. \textit{Right:} A DAG depicting the Structural Causal Model of the prediction function $f$.
The model $f$ only relies on the inputs corresponding to $X_1$ and $X_2$ for its prediction, here denoted as $\underline{X}_1$ and $\underline{X}_2$ respectively. Although the feature  $\underline{X}_3$ is not directly being used by the model, the prediction $\hat{Y}$ depends on $X_3$ via variable $X_2$.
 (b) Permutation Feature Importance (PFI) (direct importance) and XXX (indirect observational importance). We can see that in combination the two methods allow to infer that $X_3$ only influences the performance indirectly, whereas $X_1$ and $X_2$ are directly being used. }
\label{fig:dag-motivation-old} 
\end{figure}

==> figures/old/dag-motivation.tex <==
\begin{figure}[!htb]
\centering
\subfigure[DAG]{
	\begin{tikzpicture}[thick, scale=1.3, every node/.style={scale=0.8, line width=0.3mm, black, fill=white}]
		%

		\draw[dotted] (-1.3,-1.25) -- (.3,-1.25) -- (.3,1.25) -- (-1.3,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (x1) at (0, 1) {$X_1$};
		\node[draw, circle, scale=0.7] (x2) at (0, 0) {$X_2$};
		\node[draw, circle, scale=0.7] (x3) at (0, -1) {$X_3$};
		\node[draw, circle, scale=0.7] (y) at (-1, .5) {$Y$};
		\node[scale=0.7] (dots) at (-.5, -1.5) {data level, variables};
		
		\draw[dotted] (.7,-1.25) -- (2.3,-1.25) -- (2.3,1.25) -- (.7,1.25) -- cycle;
		\node[draw, circle, scale=0.7] (ux1) at (1, 1) {$\underline{X}_1$};
		\node[draw, circle, scale=0.7] (ux2) at (1, 0) {$\underline{X}_2$};
		\node[draw, circle, scale=0.7] (yhat) at (2, .5) {$\hat{Y}$};
		\node[scale=0.7] (dots) at (1.5,-1.5) {model level, features};
		
		\draw[-] (x1) -- (y);
		\draw[->] (x3) -- (y);
		\draw[->] (x2) -- (x3);
		\draw[->,gray] (x1) -- (ux1);
		\draw[->,gray] (x2) -- (ux2);
		\draw[->] (ux1) -- (yhat);
		\draw[->] (ux2) -- (yhat);
	
	\end{tikzpicture}
	
}
\subfigure[Direct and Total (obs.) Importance]{
\includegraphics[width=0.5\textwidth]{figures/relevance_types_direct_vs_total}
}
\caption{A linear OLS regression model was fit on $D = \{\underline{X}_1, \underline{X}_2\}$ to predict $Y$. (a) \textit{Left:} A causal DAG depicting the underlying data generating mechanism. All relationships are linear with Gaussian noise. \textit{Right:} A DAG depicting the Structural Causal Model of the prediction function $f$.
The model $f$ only relies on the inputs corresponding to $X_1$ and $X_2$ for its prediction, here denoted as $\underline{X}_1$ and $\underline{X}_2$ respectively. Although the feature  $\underline{X}_3$ is not directly being used by the model, the prediction $\hat{Y}$ is indirectly associated with $X_3$ via variable $X_2$.
 (b) Permutation Feature Importance (PFI) (direct importance) and XXX (indirect observational importance). We can see that in combination the two methods allows to infer that $X_3$ only influences the performance indirectly, whereas $X_1$ and $X_2$ are directly being used. However, it remains unclear via which feature $X_3$ indirectly influences the prediction.}
\label{fig:dag-motivation} 
\end{figure}

==> figures/old/notation-overview.tex <==
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[thick, scale=.9, every node/.style={scale=0.8, line width=0.3mm, black, fill=white}]
		%
		\draw[fill=green, opacity=0.3, draw opacity=0.0] (-1.5,0) circle (0.4cm);
		\draw[fill=green, opacity=0.3, draw opacity=0.0] (0,0) circle (1cm);
		\draw[fill=orange, opacity=0.3, draw opacity=0.0] (1,0) circle (0.75cm);
		%\draw[fill=purple, opacity=0.3] (0.75,-0.75) circle (0.6cm);
		
		
		\node[font=\large, fill opacity=0.0, text opacity=1.0] (xj) at  (-1.5,-0.65) {$\{j\}$};
		\node[font=\large, fill opacity=0.0, text opacity=1.0] (R) at  (0,-1.25) {$R$};
		\node[font=\large, fill opacity=0.0, text opacity=1.0] (uR) at  (-0.25,-.04) {$\underline{R}$};
		\node[font=\large, fill opacity=0.0, text opacity=1.0] (G) at  (1,-1) {$G$};
		\node[font=\large, fill opacity=0.0, text opacity=1.0] (Gstar) at  (1.35,0) {$G^*$};
		\node[font=\large, fill opacity=0.0, text opacity=1.0] (oG) at  (.7,.04){$\overline{G}$};

		%
	\end{tikzpicture}
	\caption{Overview of our notation.}
\label{fig:scm-data-model} 
\end{figure}

==> latex-math/basic-math.tex <==
% math spaces
\ifdefined\N                                                                % N, naturals
\renewcommand{\N}{\mathds{N}}                                                % N defined by "siunitx" (which we use), for "NEWTON"
\else
  \newcommand{\N}{\mathds{N}}
\fi
\newcommand{\Z}{\mathds{Z}}                                                 % Z, integers
\newcommand{\Q}{\mathds{Q}}                                                 % Q, rationals
\newcommand{\R}{\mathds{R}}                                                 % R, reals
\ifdefined\C
  \renewcommand{\C}{\mathds{C}}                                             % C, complex
\else
  \newcommand{\C}{\mathds{C}}
\fi
\newcommand{\HS}{H}                                               % H, hilbertspace
\newcommand{\continuous}{\mathcal{C}}                                       % C, space of continuous functions
\newcommand{\M}{\mathcal{M}} 												% machine numbers
\newcommand{\epsm}{\epsilon_m} 												% maximum error

% counting / finite sets
\newcommand{\setn}{\{1, \ldots, n\}} 											% {1, ..., n}
\newcommand{\setp}{\{1, \ldots, p\}}											% {1, ..., p}
\newcommand{\setg}{\{1, \ldots, g\}}											% {1, ..., g}
\newcommand{\setzo}{\{0, 1\}} 		        			    				% {0, 1}
\newcommand{\setmp}{\{-1, +1\}}     				    					% {-1, 1}


% basic math stuff
\newcommand{\xt}{\tilde x}													% x tilde
\def\argmax{\mathop{\sf arg\,max}}                                          % argmax
\def\argmin{\mathop{\sf arg\,min}}                                          % argmin
\newcommand{\sign}{\operatorname{sign}}                                     % sign, signum
\newcommand{\I}{\mathbb{I}}                                                 % I, indicator
\newcommand{\order}{\mathcal{O}}                                            % O, order
\newcommand{\fp}[2]{\frac{\partial #1}{\partial #2}}                        % partial derivative
\newcommand{\pd}[2]{\frac{\partial{#1}}{\partial #2}}						% partial derivative

% sums and products
\newcommand{\sumin}{\sum\limits_{i=1}^n}											% summation from i=1 to n
\newcommand{\sumjp}{\sum\limits_{j=1}^p}											% summation from j=1 to p
\newcommand{\sumik}{\sum\limits_{i=1}^k}											% summation from i=1 to k
\newcommand{\sumkg}{\sum\limits_{k=1}^g}											% summation from k=1 to g
\newcommand{\sumjg}{\sum\limits_{j=1}^g}											% summation from j=1 to g
\newcommand{\meanin}{\frac{1}{n} \sum\limits_{i=1}^n}			    				% mean from i=1 to n
\newcommand{\meankg}{\frac{1}{g} \sum\limits_{k=1}^g}			    				% mean from k=1 to g
\newcommand{\prodin}{\prod\limits_{i=1}^n}											% product from i=1 to n
\newcommand{\prodkg}{\prod\limits_{k=1}^g}											% product from k=1 to g
\newcommand{\prodjp}{\prod\limits_{j=1}^p}											% product from j=1 to p

% linear algebra
\newcommand{\one}{\boldsymbol{1}}                                           % 1, unitvector
\newcommand{\zero}{\mathbf{0}}													% 0-vector
\newcommand{\id}{\boldsymbol{I}}                                                % I, identity
\newcommand{\diag}{\operatorname{diag}}                                     % diag, diagonal
\newcommand{\trace}{\operatorname{tr}}                                      % tr, trace
\newcommand{\spn}{\operatorname{span}}                                      % span
\newcommand{\scp}[2]{\left\langle #1, #2 \right\rangle}                     % <.,.>, scalarproduct
\newcommand{\mat}[1]{ 														% short pmatrix command
	\begin{pmatrix}
		#1
	\end{pmatrix}
}
\newcommand{\Amat}{\mathbf{A}}													% matrix A
\newcommand{\xv}{\mathbf{x}}													% vector x (bold)
\newcommand{\yv}{\mathbf{y}}													% vector y (bold)
\newcommand{\Deltab}{\mathbf{\Delta}}											% error term for vectors


% basic probability + stats
\renewcommand{\P}{\mathds{P}}                                               % P, probability
\newcommand{\E}{\mathds{E}}                                                 % E, expectation
\newcommand{\var}{\mathsf{Var}}                                             % Var, variance
\newcommand{\cov}{\mathsf{Cov}}                                             % Cov, covariance
\newcommand{\corr}{\mathsf{Corr}}                                           % Corr, correlation
\newcommand{\normal}{\mathcal{N}}                                           % N of the normal distribution
\newcommand{\iid}{\overset{i.i.d}{\sim}}                                    % dist with i.i.d superscript
\newcommand{\distas}[1]{\overset{#1}{\sim}}                                 % ... is distributed as ...


==> latex-math/ml-automl.tex <==


% lambdav
\newcommand{\lambdav}{\bm{\lambda}}											% lambda vector



==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(x)}                    % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)}          % ambiguity/instability of ensemble


==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{r^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{r^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-feature-sel.tex <==
% ml - feature selection

\newcommand{\xjNull}{x_{j_0}}
\newcommand{\xjEins}{x_{j_1}}
\newcommand{\xl}{\mathbf{x}_l}
\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax}

==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(\bm{x}), k\left(\bm{x}, \bm{x}^\prime\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\mathbf{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\mathbf{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-mbo.tex <==
% ml - MBO
\newcommand{\sxh}{\hat{s}(x)} % uncertainty shat(x)
\newcommand{\vxh}{\hat{s}^2(x)}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\kstarx}{\mathbf{k}_*(x)}
\newcommand{\xpi}[1][i]{x^{*(#1)}}
\newcommand{\vhx}{\ensuremath{\sh^2(\xv)}\xspace}          % local estimated variance at point x
\newcommand{\shx}{\ensuremath{\sh(\xv)}\xspace}            % local estimated uncertainty at point x
\newcommand{\sh}{\ensuremath{\hat{s}}\xspace}              % local estimated uncertainty
\newcommand{\px}{\ensuremath{\boldsymbol{x}^*}}
\newcommand{\equote}[1]{``#1''}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\yx}{\ensuremath{y(\vecx)}}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}           % domain / search space

% already defined in basic-math:
% \newcommand{\yv}{\boldsymbol{y}}
\newcommand{\fhx}{\ensuremath{\fh(\xv)}\xspace}            % surrogate (x), better use \mhx for predicted value



\newcommand{\minit}{m_{\text{init}}}											% Size of the initial design
\newcommand{\lambdai}{\lambdab^{[i]}}											% input for black box optimization 
\newcommand{\lambdanew}{\lambdab^{\text{new}}}								% new proposed configuration
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\lambdab^{[1]}, ..., \lambdab^{[\minit]}}  % Vector of different inputs
\newcommand{\lambdab}{\boldsymbol{\lambda}}									% input 
\newcommand{\lambdaopt}{\lambdab^{*}}											% Minimum of the black box function Psi


==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}

==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
% \newcommand{\HS}{\mathcal{H}}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}

==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  

